Beta Distribution Drift Detection for Adaptive Classifiers

With today's abundant streams of data, the only constant we can rely on is change. For stream classification algorithms, it is necessary to adapt to concept drift. This can be achieved by monitoring the model error, and triggering counter measures as changes occur. In this paper, we propose a drift detection mechanism that fits a beta distribution to the model error, and treats abnormal behavior as drift. It works with any given model, leverages prior knowledge about this model, and allows to set application-specific confidence thresholds. Experiments confirm that it performs well, in particular when drift occurs abruptly.

==> table_bitstream_abrupt.tex <==

\begin{table}[ht]
\centering
\caption{Results on the Bit-Stream Abrupt dataset.}
\label{tab:bstreamabrupt}
\scriptsize
\begin{tabular}{p{1cm}p{0.5cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}
\hline
\multirow{2}{*}{Algorithm} &       & \multicolumn{3}{c}{600 bits between changes}                                                                                                                                                     & \multicolumn{3}{c}{1,000 bits between changes}                                                                                                                                                   \\ \cline{3-8} 
                           &       & \hspace{4pt}{[}0.1, 0.3{]}                                                 & \hspace{4pt}{[}0.3, 0.5{]}                                                 & \hspace{4pt}{[}0.5, 0.7{]}                                                 & \hspace{4pt}{[}0.1, 0.3{]}                                                 & \hspace{4pt}{[}0.3, 0.5{]}                                                 & \hspace{4pt}{[}0.5, 0.7{]}                                                 \\ \hline
DDM                        & FPR   & \begin{tabular}[c]{@{}c@{}}0.0308\\   ($\pm$ 0.0201)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0186  \\ ($\pm$ 0.0106)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0167}\\   ($\pm$ 0.0152)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0102}\\   ($\pm$ 0.0069)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0058}\\   ($\pm$ 0.0037)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0085}\\   ($\pm$ 0.0044)\end{tabular} \\ \cline{2-8} 
                           & FNR   & \begin{tabular}[c]{@{}c@{}}0.5055\\   ($\pm$ 0.1813)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.2395\\   ($\pm$ 0.1555)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.4589\\   ($\pm$ 0.1869)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1710\\   ($\pm$ 0.1708)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} \\ \cline{2-8} 
                           & Delay & \begin{tabular}[c]{@{}c@{}}0.6009\\   ($\pm$ 0.2879)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.3080\\   ($\pm$ 0.1487)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0286\\   ($\pm$ 0.0436)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.6422\\   ($\pm$ 1.1461)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.5260\\   ($\pm$ 0.4517)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.4357\\   ($\pm$ 0.1016)\end{tabular} \\ \hline
EDDM                       & FPR   & \begin{tabular}[c]{@{}c@{}}0.1436\\   ($\pm$ 0.0524)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1830\\   ($\pm$ 0.0668)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.2118\\   ($\pm$ 0.0398)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0874\\   ($\pm$ 0.0327)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1022\\   ($\pm$ 0.0319)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1181\\   ($\pm$ 0.0256)\end{tabular} \\ \cline{2-8} 
                           & FNR   & \begin{tabular}[c]{@{}c@{}}0.4496\\   ($\pm$ 0.1495)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1051\\   ($\pm$ 0.1529)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.4843\\   ($\pm$ 0.1428)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1065\\   ($\pm$ 0.1567)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} \\ \cline{2-8} 
                           & Delay & \begin{tabular}[c]{@{}c@{}}0.3579\\   ($\pm$ 0.2031)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.3919\\   ($\pm$ 0.1460)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0310\\   ($\pm$ 0.0511)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.1299\\   ($\pm$ 0.8267)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.5210\\   ($\pm$ 0.3435)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.2476\\   ($\pm$ 0.2403)\end{tabular} \\ \hline
\bdd \textsubscript{20}             & FPR   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0152}\\   ($\pm$ 0.0158)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0216}\\   ($\pm$ 0.0206)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0268\\   ($\pm$ 0.0181)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0212\\   ($\pm$ 0.0109)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0234\\   ($\pm$ 0.0080)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0202\\   ($\pm$ 0.0084)\end{tabular} \\ \cline{2-8} 
\multicolumn{1}{l}{}       & FNR   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0787}\\   ($\pm$ 0.0743)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0388}\\   ($\pm$ 0.0539)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} \\ \cline{2-8} 
\multicolumn{1}{l}{}       & Delay & \begin{tabular}[c]{@{}c@{}}\textbf{0.0068}\\   ($\pm$ 0.0206)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0552}\\   ($\pm$ 0.1549)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.0000}\\   ($\pm$ 0.0000)\end{tabular} \\ \hline
\end{tabular}
\end{table}

==> table_bitstream_incremental.tex <==
\begin{table}[ht]
\centering
\caption{Results on Bit-Stream Gradual dataset. TP counts the number of detected drifts in the change-phase (Maximum feasible: 150).}
\label{tab:bstreaminc}
\scriptsize
\begin{tabular}{p{1cm}p{0.5cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}}
\hline
\multirow{2}{*}{Algorithm}          &       & \multicolumn{3}{c}{First drift at instance \#10,000}                                                                                                                                                & \multicolumn{3}{c}{First drift at instance \#40,000}                                                                                                                                                 \\ \cline{3-8} 
                                    &       & $\hspace{2.5mm} 3 \cdot 10^{-4}$                                                             & $\hspace{2.5mm} 6 \cdot 10^{-4}$                                                              & $\hspace{2.5mm} 9 \cdot 10^{-4}$                                                             & $\hspace{2.5mm} 3 \cdot 10^{-4}$                                                              & $\hspace{2.5mm} 6 \cdot 10^{-4}$                                                             & $\hspace{2.5mm} 9 \cdot 10^{-4}$                                                             \\ \hline
DDM                                 & FPR   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0293}\\   ($\pm$ 0.0191)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0293}\\   ($\pm$ 0.0184)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0313}\\   ($\pm$ 0.0277)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0082}\\   ($\pm$ 0.0057)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}\textbf{0.0062}\\   ($\pm$ 0.0042)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0085}\\   ($\pm$ 0.0081)\end{tabular}   \\ \cline{2-8} 
                                    & TP    & \begin{tabular}[c]{@{}c@{}}2.1000\\   ($\pm$ 1.9891)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.6667\\   ($\pm$ 1.5563)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.8667\\   ($\pm$ 1.9619)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.5667\\   ($\pm$ 2.1242)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}2.3667\\   ($\pm$ 1.8526)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.6667\\   ($\pm$ 1.6799)\end{tabular}   \\ \cline{2-8} 
                                    & Delay & \begin{tabular}[c]{@{}c@{}}70.5909\\   ($\pm$ 44.5356)\end{tabular} & \begin{tabular}[c]{@{}c@{}}53.1481\\   ($\pm$ 32.5710)\end{tabular} & \begin{tabular}[c]{@{}c@{}}41.6207\\   ($\pm$ 23.9474)\end{tabular} & \begin{tabular}[c]{@{}c@{}}78.4444\\   ($\pm$ 28.7484)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}61.9130\\   ($\pm$ 29.3893)\end{tabular} & \begin{tabular}[c]{@{}c@{}}56.4615\\   ($\pm$ 37.4106)\end{tabular} \\ \hline
EDDM                                & FPR   & \begin{tabular}[c]{@{}c@{}}0.3100\\   ($\pm$ 0.1990)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.2867\\   ($\pm$ 0.2176)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.3080\\   ($\pm$ 0.2292)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.1190\\   ($\pm$ 0.1367)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0.0997\\   ($\pm$ 0.0866)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0900\\   ($\pm$ 0.0833)\end{tabular}   \\ \cline{2-8} 
                                    & TP    & \begin{tabular}[c]{@{}c@{}}21.5667\\   ($\pm$ 15.8213)\end{tabular} & \begin{tabular}[c]{@{}c@{}}27.6667\\   ($\pm$ 14.0056)\end{tabular} & \begin{tabular}[c]{@{}c@{}}28.2000\\   ($\pm$ 11.3325)\end{tabular} & \begin{tabular}[c]{@{}c@{}}11.5667\\   ($\pm$ 11.4154)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}18.1667\\   ($\pm$ 10.9090)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.2333\\   ($\pm$ 9.5662)\end{tabular}  \\ \cline{2-8} 
                                    & Delay & \begin{tabular}[c]{@{}c@{}}58.5000\\   ($\pm$ 34.3596)\end{tabular} & \begin{tabular}[c]{@{}c@{}}35.5333\\   ($\pm$ 20.7457)\end{tabular} & \begin{tabular}[c]{@{}c@{}}25.3333\\   ($\pm$ 15.1158)\end{tabular} & \begin{tabular}[c]{@{}c@{}}110.9600\\   ($\pm$ 28.3019)\end{tabular} & \begin{tabular}[c]{@{}c@{}}77.3000\\   ($\pm$ 21.1473)\end{tabular} & \begin{tabular}[c]{@{}c@{}}60.8333\\   ($\pm$ 17.4415)\end{tabular} \\ \hline
\bdd\textsubscript{1.5}                     & FPR   & \begin{tabular}[c]{@{}c@{}}0.0520\\   ($\pm$ 0.0271)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0480\\   ($\pm$ 0.0234)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0467\\   ($\pm$ 0.0284)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0522\\   ($\pm$ 0.0131)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0.0532\\   ($\pm$ 0.0140)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0577\\   ($\pm$ 0.0114)\end{tabular}   \\ \cline{2-8} 
\multicolumn{1}{l}{}                & TP    & \begin{tabular}[c]{@{}c@{}}9.3667\\   ($\pm$ 2.6266)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}10.8333\\   ($\pm$ 1.8988)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}11.8333\\   ($\pm$ 2.4506)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}9.2667\\   ($\pm$ 2.4212)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}10.8333\\   ($\pm$ 2.5177)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}11.9333\\   ($\pm$ 2.7681)\end{tabular}  \\ \cline{2-8} 
\multicolumn{1}{l}{}                & Delay & \begin{tabular}[c]{@{}c@{}}12.3667\\   ($\pm$ 10.2192)\end{tabular} & \begin{tabular}[c]{@{}c@{}}9.1000\\   ($\pm$ 7.1757)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}9.0333\\   ($\pm$ 10.0945)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}9.9333\\   ($\pm$ 8.8164)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}11.7667\\   ($\pm$ 11.1615)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.9333\\   ($\pm$ 12.3530)\end{tabular}  \\ \hline
\multicolumn{1}{l}{\bdd\textsubscript{1.1}} & FPR   & \begin{tabular}[c]{@{}c@{}}0.1267\\   ($\pm$ 0.0404)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.1120\\   ($\pm$ 0.0329)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.1173\\   ($\pm$ 0.0345)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.1705\\   ($\pm$ 0.0236)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0.1667\\   ($\pm$ 0.0194)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.1647\\   ($\pm$ 0.0162)\end{tabular}   \\ \cline{2-8} 
\multicolumn{1}{l}{}                & TP    & \begin{tabular}[c]{@{}c@{}}\textbf{36.1667}\\   ($\pm$ 4.0586)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{45.5000}\\   ($\pm$ 3.4617)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{55.6333}\\   ($\pm$ 2.9831)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{35.6000}\\   ($\pm$ 2.9732)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{46.4000}\\   ($\pm$ 3.3625)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{54.8667}\\   ($\pm$ 3.4903)\end{tabular}  \\ \cline{2-8} 
\multicolumn{1}{l}{}                & Delay & \begin{tabular}[c]{@{}c@{}}\textbf{3.1333}\\   ($\pm$ 3.1170)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{3.4333}\\   ($\pm$ 4.1528)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{2.7667}\\   ($\pm$ 2.4315)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{3.6333}\\   ($\pm$ 3.5729)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}\textbf{3.4000}\\   ($\pm$ 2.7761)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{2.6000}\\   ($\pm$ 2.4440)\end{tabular}   \\ \hline
\end{tabular}
\end{table}

==> table_bitstream_incremental_autodecay.tex <==
\begin{table}[ht]
\scriptsize
\centering
\caption{Results on Bit-Stream Gradual dataset. TP counts the number of detected drifts in the change-phase (Maximum feasible: 150).}
\label{tab:bstreaminc}
\begin{tabular}{p{1cm}p{0.5cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}}
\hline
\multirow{2}{*}{Algorithm}          &       & \multicolumn{3}{c}{First drift at instance \#10,000}                                                                                                                                                & \multicolumn{3}{c}{First drift at instance \#40,000}                                                                                                                                                 \\ \cline{3-8} 
                                    &       & $\hspace{2.5mm} 3 \cdot 10^{-4}$                                                             & $\hspace{2.5mm} 6 \cdot 10^{-4}$                                                              & $\hspace{2.5mm} 9 \cdot 10^{-4}$                                                             & $\hspace{2.5mm} 3 \cdot 10^{-4}$                                                              & $\hspace{2.5mm} 6 \cdot 10^{-4}$                                                             & $\hspace{2.5mm} 9 \cdot 10^{-4}$                                                             \\ \hline
DDM                                 & FPR   & \begin{tabular}[c]{@{}c@{}}0.0320\\   ($\pm$ 0.0208)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0328\\   ($\pm$ 0.0265)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0296\\   ($\pm$ 0.0201)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0065}\\   ($\pm$ 0.0065)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}\textbf{0.0071}\\   ($\pm$ 0.0057)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0085}\\   ($\pm$ 0.0052)\end{tabular}   \\ \cline{2-8} 
                                    & TP    & \begin{tabular}[c]{@{}c@{}}1.9200\\   ($\pm$ 2.0282)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.0800\\   ($\pm$ 2.7989)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.0200\\   ($\pm$ 1.8275)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.4800\\   ($\pm$ 1.5651)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}2.0800\\   ($\pm$ 1.8203)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.6200\\   ($\pm$ 1.9585)\end{tabular}   \\ \cline{2-8} 
                                    & Delay & \begin{tabular}[c]{@{}c@{}}67.7742\\   ($\pm$ 33.7846)\end{tabular} & \begin{tabular}[c]{@{}c@{}}52.9091\\   ($\pm$ 35.4778)\end{tabular} & \begin{tabular}[c]{@{}c@{}}48.5532\\   ($\pm$ 32.3582)\end{tabular} & \begin{tabular}[c]{@{}c@{}}69.8966\\   ($\pm$ 26.9320)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}72.6410\\   ($\pm$ 41.4899)\end{tabular} & \begin{tabular}[c]{@{}c@{}}59.4884\\   ($\pm$ 31.4985)\end{tabular} \\ \hline
EDDM                                & FPR   & \begin{tabular}[c]{@{}c@{}}0.3072\\   ($\pm$ 0.2094)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.2912\\   ($\pm$ 0.2425)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.3180\\   ($\pm$ 0.2062)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0949\\   ($\pm$  0.0896)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0.0887\\   ($\pm$ 0.0955)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0817\\   ($\pm$ 0.0870)\end{tabular}   \\ \cline{2-8} 
                                    & TP    & \begin{tabular}[c]{@{}c@{}}\textbf{20.5600}\\   ($\pm$ 15.9062)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{26.1600}\\   ($\pm$ 14.3169)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{32.8600}\\   ($\pm$ 12.2622)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{11.9600}\\   ($\pm$ 11.3066)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{15.7000}\\   ($\pm$ 11.9034)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{20.6000}\\   ($\pm$ 9.7160)\end{tabular}  \\ \cline{2-8} 
                                    & Delay & \begin{tabular}[c]{@{}c@{}}53.1800\\   ($\pm$ 37.0063)\end{tabular} & \begin{tabular}[c]{@{}c@{}}41.4000\\   ($\pm$ 18.7979)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{24.6800}\\   ($\pm$ 15.1966)\end{tabular} & \begin{tabular}[c]{@{}c@{}}102.4773\\   ($\pm$ 38.1680)\end{tabular} & \begin{tabular}[c]{@{}c@{}}85.1400\\   ($\pm$ 21.7642)\end{tabular} & \begin{tabular}[c]{@{}c@{}}62.2000\\   ($\pm$ 19.0379)\end{tabular} \\ \hline
\bdd                     & FPR   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0220}\\   ($\pm$ 0.0220)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0144}\\   ($\pm$ 0.0160)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}\textbf{0.0196}\\   ($\pm$ 0.0162)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.0160\\   ($\pm$ 0.0084)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0.0176\\   ($\pm$ 0.0093)\end{tabular}   & \begin{tabular}[c]{@{}c@{}} 0.0157\\   ($\pm$ 0.0077)\end{tabular}   \\ \cline{2-8} 
\multicolumn{1}{l}{}                & TP    & \begin{tabular}[c]{@{}c@{}}3.1200\\   ($\pm$ 1.4918)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.1800\\   ($\pm$ 1.5961)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}3.5600\\   ($\pm$ 1.7682)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}3.1400\\   ($\pm$ 1.2651)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}3.1400\\   ($\pm$ 1.6001)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}3.8000\\   ($\pm$ 1.6000)\end{tabular}  \\ \cline{2-8} 
\multicolumn{1}{l}{}                & Delay & \begin{tabular}[c]{@{}c@{}}\textbf{37.7292}\\   ($\pm$ 34.6023)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{35.3125}\\   ($\pm$ 29.6396)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}31.4898\\   ($\pm$ 28.4103)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{34.1250}\\   ($\pm$ 27.7636)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}\textbf{33.3750}\\   ($\pm$ 31.4912)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{25.6939}\\   ($\pm$ 20.0145)\end{tabular}  \\ \hline
\end{tabular}
\end{table}

==> table_elec.tex <==
\begin{table}[ht]
\centering
\caption{Results on the Elec2 dataset}
\label{tab:elec}
\scriptsize
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{c}{} & No Detector & DDM    & EDDM   & \bdd\textsubscript{1.1}  & \bdd\textsubscript{5}  & \bdd\textsubscript{10}  & \bdd\textsubscript{20}  \\
Accuracy             & 0.7270      & 0.7233 & 0.7244 & \textbf{0.7381}    & 0.7302  & 0.7290   & 0.7265   \\ \hline
\end{tabular}
\end{table}

==> table_synth_datasets.tex <==
\begin{table}[ht]
\centering
\caption{Results on synthetic datasets}
\label{tab:synth}
\scriptsize
%\begin{tabular}{p{1cm}p{0.5cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}}
\begin{tabular}{cccc|ccc}
\hline
\multirow{2}{*}{Algorithm}      & \multicolumn{3}{c}{SEA Concepts}                                                                                                                                                                          & \multicolumn{3}{c}{Rotating Hyperplane}                                                                                                                                                         \\ \cline{2-7} 
                                & 0.0                                                            & 0.1                                                            & 0.2                                                            & 10                                                             & 30                                                             & 60                                                             \\ \hline
\multicolumn{1}{l}{No Detector} & \begin{tabular}[c]{@{}c@{}}0.9133\\ ($\pm$ 0.0013)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.8479 \\ ($\pm$ 0.0014)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.7633  \\ ($\pm$ 0.0013)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.6143\\   ($\pm$ 0.0074)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.5936\\   ($\pm$ 0.0110)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.5734\\   ($\pm$ 0.0117)\end{tabular} \\ \cline{2-7} 
DDM                             & \begin{tabular}[c]{@{}c@{}}0.9452 \\ ($\pm$ 0.0085)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.8662\\  ($\pm$ 0.0108)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.7673\\   ($\pm$ 0.0101)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9302\\   ($\pm$ 0.0086)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9048\\   ($\pm$ 0.0110)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8682\\   ($\pm$ 0.0110)\end{tabular} \\ \cline{2-7} 
EDDM                            & \begin{tabular}[c]{@{}c@{}}0.9463\\  ($\pm$ 0.0025)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.8617\\  ($\pm$ 0.0039)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.7605\\   ($\pm$ 0.0036)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9394\\   ($\pm$ 0.0061)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9098\\   ($\pm$ 0.0104)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8793\\   ($\pm$ 0.0109)\end{tabular} \\ \cline{2-7} 
\bdd                            & \begin{tabular}[c]{@{}c@{}}\textbf{0.9503}\\   ($\pm$ 0.0030)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.8723}\\   ($\pm$ 0.0024)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.7739}\\   ($\pm$ 0.0059)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.9429}\\   ($\pm$ 0.0048)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.9140}\\   ($\pm$ 0.0082)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.8905}\\   ($\pm$ 0.0079)\end{tabular} \\ \hline
\end{tabular}
\end{table}
